RTAMT: Online Robustness Monitors from STL

We present RTAMT, an online monitoring library for Signal Temporal Logic (STL) and its interface-aware variant (IA-STL), providing both discrete- and dense-time interpretation of the logic. We also introduce RTAMT4ROS, a tool that integrates RTAMT with Robotic Operating System (ROS), a common environment for developing robotic applications. We evaluate RTAMT and RTAMT4ROS on two robotic case studies.

==> rtamt4ros.tex <==
\section{Scripts}
\label{sec:rtamt4ros}

\subsection{STL Monitor for ROS}
\label{sec:rtamt4ros}


\lstinputlisting{listings/rtamt4ros.txt}

\section{MATLAB Script Integrating RTAMT STL Monitor}

\lstinputlisting{listings/monitor.m}

\section{MATLAB Script for Sensitivity Analysis}
\lstinputlisting{listings/sensitivity_analysis_demo.m}

\section{MATLAB Script for Falsification Testing}
\lstinputlisting{listings/search_based_testing_demo.m}
\lstinputlisting{listings/ofun.m}
\lstinputlisting{listings/outfun.m}

\section{MATLAB Level 2 S-Function for STL Online Monitors}
\lstinputlisting{listings/online_monitor.m}

